Minimax Optimal Rates for Poisson Inverse Problems with Physical Constraints

This paper considers fundamental limits for solving sparse inverse problems in the presence of Poisson noise with physical constraints. Such problems arise in a variety of applications, including photon-limited imaging systems based on compressed sensing. Most prior theoretical results in compressed sensing and related inverse problems apply to idealized settings where the noise is i.i.d., and do not account for signal-dependent noise and physical sensing constraints. Prior results on Poisson compressed sensing with signal-dependent noise and physical constraints provided upper bounds on mean squared error performance for a specific class of estimators. However, it was unknown whether those bounds were tight or if other estimators could achieve significantly better performance. This work provides minimax lower bounds on mean-squared error for sparse Poisson inverse problems under physical constraints. Our lower bounds are complemented by minimax upper bounds. Our upper and lower bounds reveal that due to the interplay between the Poisson noise model, the sparsity constraint and the physical constraints: (i) the mean-squared error does not depend on the sample size $n$ other than to ensure the sensing matrix satisfies RIP-like conditions and the intensity $T$ of the input signal plays a critical role; and (ii) the mean-squared error has two distinct regimes, a low-intensity and a high-intensity regime and the transition point from the low-intensity to high-intensity regime depends on the input signal $f^*$. In the low-intensity regime the mean-squared error is independent of $T$ while in the high-intensity regime, the mean-squared error scales as $\frac{s \log p}{T}$, where $s$ is the sparsity level, $p$ is the number of pixels or parameters and $T$ is the signal intensity.

==> NISLAB_macros.tex <==
\usepackage{mathrsfs}
\usepackage{amsmath,amssymb,latexsym}
\usepackage{amsfonts}
\usepackage{times,lastpage,bm,xspace,subfigure}
\usepackage{bibunits}
\usepackage{mathrsfs,bbm}
\usepackage{dsfont}
\usepackage{graphicx}
\RequirePackage{color}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{stmaryrd}
% Example definitions.
% --------------------

% === ZTH Macros ====
% reals, for the reals!
\newcommand{\reals}{\ensuremath{\mathds{R}}}
% diag, for diagonal matrices
%\DeclareMathOperator{\diag}{diag}
% bdiag, for block diagonal matrices
\DeclareMathOperator{\bdiag}{bdiag}
% soft, for soft threshold
\DeclareMathOperator{\soft}{soft}
% sgn, for signum function
\DeclareMathOperator{\sgn}{sgn}
% arg min, note the * places subscripts/superscripts in the limit positions
\DeclareMathOperator*{\argmin}{arg\,min}
% arg min, note the * places subscripts/superscripts in the limit positions
\DeclareMathOperator*{\argmax}{arg\,max}
% Minimize
\DeclareMathOperator*{\minimize}{minimize}
% Subject to
\DeclareMathOperator*{\st}{subject\ to}
% Script L for Lagrangian
\def\L{{\cal L}}


\def\Risk#1#2{R\left( #1, #2\right)} % L1 risk
 \def\tf{f^*}





\def\x{{\mathbf x}}
\def\Re{\mathbb{R}}
\def\expect{\mathbb{E}}
\def\ones{\mathbbm{1}}
\newcommand{\ints}{{\mathbb{Z}}}
\def \Poisson{{{\rm Poisson}}}
\def\deq{\triangleq}
\def\hf{\widehat{f}}
\def\ftrue{f^{\star}}
\def\ttheta{\theta^{\star}}
\def\htheta{\widehat{\theta}}
\def\argmin{\mathop{\!\arg \min}}
\def\grad{\nabla}
\def\tepsilon{\tilde{\epsilon}}
\def\S{\mathcal{S}}
\def\pen{{\rm pen}}
\def\sP{\mathcal P}
\def\th{^{\rm th}}
\def\bI{\mathbb{I}}

\newenvironment{squishlist}
{   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{2pt}      \setlength{\parsep}{2pt}
      \setlength{\topsep}{0pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }
      {\end{list}}

\newenvironment{myproof}
{\noindent{\sc Proof:}}
{$\square$ \\}

\usepackage{booktabs}
\newcommand{\todo}[1]{{\textcolor{red}{[#1]}}}
\newcommand{\wh}[1]{{\widehat{#1}}}
\newcommand{\wt}[1]{{\widetilde{#1}}}
%\newcommand{\st}{\;\rm~subject~to~}

\def\Prob{{\mathbb P}}



